Integrative Decoding: Improve Factuality via Implicit Self-consistency

Self-consistency-based approaches, which involve repeatedly sampling multiple outputs and selecting the most consistent one as the final response, prove to be remarkably effective in improving the factual accuracy of large language models. Nonetheless, existing methods usually have strict constraints on the task format, largely limiting their applicability. In this paper, we present Integrative Decoding (ID), to unlock the potential of self-consistency in open-ended generation tasks. ID operates by constructing a set of inputs, each prepended with a previously sampled response, and then processes them concurrently, with the next token being selected by aggregating of all their corresponding predictions at each decoding step. In essence, this simple approach implicitly incorporates self-consistency in the decoding objective. Extensive evaluation shows that ID consistently enhances factuality over a wide range of language models, with substantial improvements on the TruthfulQA (+11.2%), Biographies (+15.4%) and LongFact (+8.5%) benchmarks. The performance gains amplify progressively as the number of sampled responses increases, indicating the potential of ID to scale up with repeated sampling.

==> Figures/test_case_study.tex <==
\setlength{\columnsep}{0.2cm}


\begin{figure*}[ht]\footnotesize
\begin{tcolorbox}[colback=boxcolor!5!white,colframe=boxcolor!80!black]

Maria Sharapova is a Russian professional tennis player who has had a highly successful career in the sport. Here are some specific details and examples about her:
\vspace{\baselineskip}

\textbf{Early Life and Career}
\begin{itemize}[left=2mm]
    \item Born on April 19, 1987, in Nyagan, Russia
    \item Moved to the United States at the age of seven to pursue a tennis career
    \item Trained at the Nick Bollettieri Tennis Academy in Bradenton, Florida
    \item Turned pro in 2001 at the age of 14
\end{itemize}
\vspace{\baselineskip}
\textbf{Career Highlights}
\begin{itemize}[left=2mm]
    \item Won five Grand Slam singles titles: 2004 Wimbledon, 2012 French Open, 2012 US Open, 2014 French Open, and 2015 Australian Open
    \item Reached the finals of the Australian Open three times (2008, 2015, and 2019)
    \item Reached the finals of the French Open three times (2006, 2013, and 2014)
    \item Reached the finals of the US Open three times (2006, 2012, and 2014)
    \item Won 36 WTA singles titles, including five Premier Mandatory titles
    \item Held the world No. 1 ranking for a total of 21 weeks (2008 and 2015)
\end{itemize}
\vspace{\baselineskip}
\textbf{Notable Matches and Rivalries}
\begin{itemize}[left=2mm]
    \item Defeated Serena Williams in the 2004 Wimbledon final, becoming the first Russian woman to win the title
    \item Lost to Justine Henin in the 2008 Australian Open final
    \item Defeated Simona Halep in the 2015 French Open final
    \item Lost to Angelique Kerber in the 2016 Australian Open final
    \item Had a long-standing rivalry with Serena Williams, with whom she has played 22 times, winning 11 matches and losing 11
\end{itemize}
\vspace{\baselineskip}

\textbf{Doping Scandal}
\begin{itemize}[left=2mm]
    \item Tested positive for meldonium, a banned substance, at the 2016 Australian Open
    \item Suspended for 15 months by the International Tennis Federation (ITF) and lost her ranking and prize money
    \item Returned to professional tennis in 2017 and won the 2017 Stuttgart Open
\end{itemize}
\vspace{\baselineskip}

\textbf{Personal Life}
\begin{itemize}[left=2mm]
    \item Has been in a relationship with Sasha Vujacic, a former NBA player, since 2019
    \item Has a strong social media presence, with over 12 million followers on Instagram
    \item Involved in various charitable initiatives, including the Maria Sharapova Foundation, which supports underprivileged children and young athletes
\end{itemize}

\textbf{Awards and Recognition}
\begin{itemize}[left=2mm]
    \item Won the WTA Newcomer of the Year award in 2004
    \item Won the WTA Player of the Year award in 2012
    \item Inducted into the International Tennis Hall of Fame in 2020
\end{itemize}
\vspace{\baselineskip}

\textbf{Career Statistics}
\begin{itemize}[left=2mm]
    \item Singles wins: 655-225
    \item Singles titles: 36
    \item Grand Slam singles titles: 5
    \item Career prize money: over \$38 million
\end{itemize}

\end{tcolorbox}
\caption{The prompt utilized for generating the task-oriented synthetic data.}
\label{fig:synthetic_prompt}
\end{figure*}

==> Sections/intro_bk.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/cover_plots.pdf}
    \caption{With no need of retrieving external knowledge and additional training, integrative decoding consistently improves the factuality performance over six types of large language models, with substantial improvements on the TruthfulQA, Biographies, and LongFact datasets. }
    \label{fig:enter-label}
\end{figure}

\section{Introduction}
Despite achieving significant breakthroughs in various domains, Large Language Models (LLMs) remain notorious for their tendency to produce non-factual and erroneous content, a phenomenon commonly known as `hallucination' \citep{lewis2020retrieval, ji2023survey, zhang2023siren}. 
Previous studies found that the degree of consistency among LLMs' different outputs, often termed as `\emph{self-consistency}',\footnote{`Self-consistency' is sometimes specifically used to refer to the method proposed by \cite{wang2023self}. In this paper, we employ this term in a broader sense to denote the degree of consistency among a model's discholfferent outputs.} 
can serve as a useful indicator for addressing hallucination \citep{wang2023self,shi2022codesc,chen2023usc,thirukovalluru2024asc,malon2024scdecoding,niels2024selfcontradict}. 
Previous research indicates that the facts consistently supported by LLMs' different sampled responses are more likely to be factual, compared to those only appearing sporadically or inconsistently across multiple outputs \citep{wang2023self,manakul-etal-2023-selfcheckgpt}. 
%To address this, a research direction that has received growing attention is improving factuality of LLMs from the perspective of \emph{self-consistency} \citep{wang2022self}. 
%In a broad sense, the idea of self-consistency involves sampling multiple responses from the LLM and hypothesizing the content that has the greatest consistency across all responses as the final output. 
Several methods driven by self-consistency have been developed to improve factuality, which usually involve sampling multiple responses for the same prompt and then meticulously choosing the most self-consistent one as the final output \blue{[cite]}. More recently, \blue{[cite]} empirically demonstrated that model performance can improve almost log-linearly as the number of sampled responses increases.
\blue{scaling law?}

While showing promising results, the existing self-consistency methods generally have strict constraints on the output format, as they define `consistency' as exact matches between the answers parsed from the responses and choose the most frequent answer as the final output \citep{wang2023self}. This limits their application mainly in some short-answer tasks like arithmetic problems. 
%It is predominantly used in short-answer tasks, such as math problems and multiple-choice questions, where `consistency' between responses can be easily defined as exact matches between the answers parsed from the responses \blue{[cite]}. 
%This strategy has demonstrated huge performance leaps in these task scenarios. 
%This strategy can enable huge performance leaps in short-answer tasks (e.g., math problems and multiple-choice questions) \blue{[cite]}, where `consistency' between responses can be easily defined via exact match of the inferred answers. 
%In these tasks, the idea of self-consistency can be easily applied by extracting the inferred answer from each sampled response and then using the most frequent answer as the final output. 
In tasks where answers cannot be categorized via exact matches, such as long-form text generation, utilizing self-consistency to mitigate hallucinations becomes much more challenging. %, but it still holds considerable promise. %, such as providing a detailed explanation for queried concept or summarizing given texts.
%In fact, the idea of self-consistency in a broader sense also holds considerable promise for addressing hallucinations in long-form generation. 
%Recent studies suggest that, in a long-form generated text, the pieces of information repeatedly mentioned in multiple sampled responses are more likely to be factual than those that infrequently appear \blue{[cite]}. 
In the few works that explored this topic, they generally regard a long-form response as a series of atomic facts %\footnote{Atomic facts are defined as the simplest kinds of facts that cannot be broken down further \blue{[cite]}. For example, the sentence `\emph{Harry was born in London in 1980}' contains two atomic facts: `\emph{Harry was born in London}' and `\emph{Harry was born in 1980}'.} 
and assess their factuality via self-consistency separately \blue{[cite]}. % fine-tune for, self-contrast, atomic self-consistency
%For example, \blue{[cite]} check the factuality of each newly generated sentence by raising questions around the facts mentioned in this sentence and sampling the LLM's answers to it. If there exist inconsistency across the sampled answers, they classify this fact as unreliable and revise the sentence accordingly, before proceeding to generate the next sentence. % to repeatedly generate illustrations around the concepts mentioned in the fact under review. 
%Building upon this observation, one straightforward approach for mitigating hallucinations entails splitting each sampled response into a list of atomic facts\footnote{Atomic facts are the simplest kinds of facts that cannot be broken down further \blue{[cite]}. For example, the sentence `\emph{Harry was born in London in 1980}' contains two atomic facts: `\emph{Harry was born in London}' and `\emph{Harry was born in 1980}'.} and removing those that infrequently appear across the responses \blue{[cite]}. 
%For example, \blue{[cite]} directly removes those facts that infrequently appear across different responses by clustering them based on the semantic embeddings. 
%Nonetheless, one issue within these approaches is that the facts in one response are often interlinked and cannot be treated separately. 
%For instance, they would be impracticable if the response contains sequential reasoning. 
However, they typically rely on numerous prompting to verify if a fact is consistently supported by other sampled responses, a process that can be costly and time-consuming. %In addition, statements within a response are often interlinked and cannot be treated separately, such as in the cases where the response contains chain-of-thought reasoning \blue{[cite]}. 
%Removing one may severely disrupt the overall coherence. For instance, this approach would be impracticable if the response contains sequential reasoning. 
%However, a primary issue within this method is that there may exist logical connections between the atomic facts (i.e., one atomic fact may serve as the context or precondition for another). Directly removing one of them may cause incoherence in the text. 
%Moreover, this approach requires extensive comparisons to verify semantic equivalence among facts, with complexity escalating with the square of the number of atomic facts, making it computationally demanding. 
% for very long text. 
%as it necessitates numerous comparisons for determining whether two facts are semantically equal, whose complexity increases significantly with the square of the number of atomic facts in question. % making this approach computationally demanding. %is also challenging. Since one fact can be expressed in different ways, verifying if two facts are semantically equal is complicated. Additionally, the number of these verification operations increases exponentially with the number of atomic facts in question, making this approach computationally demanding. Moreover, measuring the frequency of each atomic fact is also challenging. Since one fact can be expressed in different ways, verifying if two facts are semantically equal is complicated. Additionally, the number of these verification operations increases exponentially with the number of atomic facts in question, making this approach computationally demanding. %the number of this equality assessment operations will rise with square of the number of atomic facts. 
%Building upon this observation, \blue{[cite]} developed a method to mitigate hallucinations effectively. They regard a long-form response as a series of atomic facts. During generation, each newly produced fact is verified for factuality by prompting the LLM to repeatedly generate illustrations around the concepts mentioned in the fact under review. If the fact is consistently supported by the triggered content, it is retained in the final response and the next atomic fact is generated following it; otherwise, this fact is modified or discarded entirely.
%Specifically, in the generation process, each newly generated fact is checked in terms of its consistency with other sampled responses from the LLM and it will be discarded if lacking strong consistency. 
%one straightforward approach for mitigating hallucinations is to 
%However, a primary issue within this method is that the generated text cannot be simply regarded as a number of individual atomic facts, as the pieces of information in a text need to rely on the context to comprehend and they may have logical connection among them. Directly removing those 
% In long-form text generation, . Recent studies on hallucination detection demonstrate. 
%However, applying self-consistency in long-form text generation is much more challenging. 
% Here, though seldom pointed out in the literature, it is in fact challenging to choose the response with the greatest challenging. 
%With the objective of extending self-consistency to various generation tasks, we ask the following question
This leads us to ask: given multiple sampled responses for the same prompt, \emph{can we directly generate a new output in a way that encourages self-consistency with all of them to improve actuality? }%the previously sampled ones?} 
\blue{polish this sentence? e.g. this example is not very accurate, but can we write it in a more vivid/insightful way like this? ``Can we encourage the self-consistent generation by implicitly voting for the most consistent responses among all potential ones?''}

\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{Figures/integrative_decoding.pdf}
\end{center}
\vspace{-3mm}
\caption{The workflow of integrative decoding: (1) sample multiple responses from the LLM; (2) form a set of new inputs by concatenating a sampled response and the original prompt; they are concurrently processed in a batch for integrative decoding, with the next token being selected by integrating all predicted logits within this batch. The final output can maintain strong overall consistency with the previously sampled responses as integrative decoding essentially incorporates self-consistency within its decoding objective (see \S\ref{sec:method}).} 
\label{fig:workflow}
\end{figure}


In this paper, we present \emph{Integrative Decoding} to achieve this. As shown in Figure \ref{fig:workflow}, the workflow of integrative decoding is simple, with no need of any additional training or external knowledge. It begins by first sampling multiple responses to the same prompt and concatenating each with this original prompt to form a new input. Each new input is preceded by a sampled responses and prompts the model to respond to the original instruction again referring to it. % following a format akin to one-shot prompting. 
These new inputs are then processed concurrently in the same batch for the model to perform the inference again. %At each decoding step, each input leads to its own predicted probability distribution for the next token. 
Crucially, instead of selecting the next token for each input independently, ID integrates the predicted logits across all inputs. The token with the highest integrated logit is selected as the next token for all inputs. Consequently, all outputs produced in this batch are identical, which is used as the final output. 
As will be explained more detailedly in Section \ref{sec:method}, such practice is able to incorporate the degree of self-consistency within the decoding objective. Intuitively, ID fosters self-consistency by allowing each input to implicitly `vote' for the next token based on a previously sampled response utilizing the in-context learning capability. \red{For example,}
%Integrative decoding can ensure the output coherence since the individual probability distributions in the batch will all favor tokens that can smoothly continue the preceding content.  Meanwhile, this strategy can also implicitly encourage self-consistency, as the power of in context learning will incline the model to repeat content in the one-shot example, which, in this case, is a response sampled in the previous step. 
%\red{For example, ...}

%2) \emph{Generality}: ID can be seamlessly applied to various generation tasks, without necessitating any task-specific adaptations. 
We evaluate integrative decoding over six types of LLMs with different scales, including LLaMA2 \citep{touvron2023llama}, LLaMA3 \citep{dubey2024llama}, Mistral-v0.2 \citep{jiang2023mistral}, Qwen2 \citep{yang2024qwen2}, Gemma2 \citep{team2024gemma}, and GLM4 \citep{glm2024chatglm}. 
We observe that integrative decoding consistently enhances the factuality of all these LLMs by a large margin on the TruthfulQA (+11.2\%), Biographies (+15.4\%) and LongFact (+8.5\%) datasets, significantly outperforming other decoding-based and ensemble-based approaches. 
Further analyses demonstrate that the performance of integrative decoding is robust to different sampling strategies and varying model scales. 
%3) \emph{Effectiveness}: our experiments demonstrate that ID can  significantly elicit factuality across a wide range of tasks over six LLMs with varying scales, including Phi-3-mini (4B parameters), Mistral-7B, Llama-3-8B, Gemma-2-9B, Gemma-2-27B, and Llama-3-70B \blue{[cite]}. We evaluate ID on both the long-form generation tasks, where the traditional self-consistency methods based on exact matches are inapplicable, such as TruthfulQA, Biography, and LongFact \blue{[cite]}, as well as the short-answer tasks like GSM8K \blue{[cite]} and AmbigQA \blue{[cite]}. \blue{The results show that ID can robustly boost performance on all these tasks.}   %include TruthfulQA \blue{[cite]}, a representative question answering dataset for measuring factuality, as well as Biography \blue{[cite]} and Longfact \blue{[cite]}, which involves biography writing and generating detailed explanations for queried concepts, respectively. Notably, the traditional self-consistency methods based on exact matches to select the answer are inapplicable in these three tasks. We also evaluate ID on several short-answer tasks where traditional self-consistency methods are feasible, including GSM8K \blue{[cite]}, AmbigQA \blue{[cite]}, and \red{XXX}. The experiments show that



==> Tables/efficiency.tex <==
\begin{minipage}[t]{0.42\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcr}
        \toprule
        \textbf{Method} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}Latency $\downarrow$ \\ (ms/token)\end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}Throughput $\uparrow$ \\ (token/s)\end{tabular}}\\
        \midrule
        Greedy & 0.10 \tiny{(×1.00)} & 975.76 \tiny{(×1.00)}$\;\;$ \\
        USC & \sethlcolor{tabcolor5}\hl{0.93 \tiny{(×9.10)}} & \sethlcolor{tabcolor5}\hl{107.73 \tiny{(×0.11)}}$\;\;$ \\
        SR & 1.97 \tiny{(×19.26)} & 50.90 \tiny{(×0.05)}$\;\;$ \\
        FSC & 1.97 \tiny{(×19.26)} & 50.88 \tiny{(×0.05)}$\;\;$ \\
        SE-SL & 8.37 \tiny{(×82.09)} & 11.96 \tiny{(×0.01)}$\;\;$ \\
        SE-RG & 7.28 \tiny{(×71.35)} & 13.74 \tiny{(×0.01)}$\;\;$ \\
        \textbf{ID} & \sethlcolor{tabcolor3}\hl{\textbf{1.13 \tiny{(×11.04)}}} & \sethlcolor{tabcolor3}\hl{\textbf{86.78 \tiny{(×0.09)}}}$\;\;$ \\
        \bottomrule
    \end{tabular}}
    \captionof{table}{Evaluation of inference efficiency. Tokens generated in intermediate steps and chain-of-thought reasoning excluded to ensure a fair comparison.}
    \label{tab:eval_efficiency}
\end{minipage}

==> Tables/eval_coherence.tex <==
\begin{minipage}[t]{0.4\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccc}
        \toprule
        \multirow{2}{*}{\textbf{Base Model}} & \multicolumn{3}{c}{\textbf{ID vs. Greedy}}\\\cmidrule(lr){2-4}
        & \multicolumn{1}{c}{\textbf{Win}  (\%)} & \multicolumn{1}{c}{\textbf{Tie}  (\%)} & \multicolumn{1}{c}{\textbf{Lose}  (\%)} \\
        \midrule
        Gemma2 & 11.95 & 80.49 & $\;\;$7.56 \\
        GLM4 & 16.34 & 72.68 & 10.98 \\
        Llama2 & 12.68 & 82.44 & $\;\;$4.88 \\
        Llama3 & $\;\;$8.54 & 82.93 & $\;\;$8.54 \\
        Mistral2 & 11.22 & 76.83 & 11.95 \\
        Qwen2 & 14.39 & 74.63 & 10.98 \\
        \bottomrule
    \end{tabular}}
    \captionof{table}{Evaluation of language coherence. The ``Win'' column indicates the ratio of cases where ID wins.}
    \label{tab:eval_coherence}
\end{minipage}

==> Tables/eval_sc.tex <==
\begin{minipage}[t]{0.56\linewidth}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{c}{\textbf{Base Model}}\\\cmidrule(lr){2-7}
        & Llama2 & Llama3 & Mistral & Qwen & Gemma & GLM \\
        \midrule
        Vanilla          & 0.6087 & 0.6323 & 0.6024 & 0.6789 & 0.7069 & 0.6453 \\
        USC              & 0.6049 & 0.6524 & 0.6064 & 0.6765 & 0.7244 & 0.6641 \\
        SR               & 0.6345 & 0.6443 & 0.6509 & 0.7195 & 0.7204 & 0.6948 \\
        FSC              & 0.5984 & 0.6343 & 0.6099 & 0.6826 & 0.7097 & 0.6795 \\
        SE-SL            & 0.6221 & 0.6715 & 0.6435 & 0.6999 & 0.7481 & 0.6725 \\
        SE-RG            & 0.6393 & 0.6466 & 0.6344 & 0.7063 & 0.7520 & 0.6809 \\
        ID & \sethlcolor{tabcolor5}\hl{\textbf{0.648}} & \sethlcolor{tabcolor5}\hl{\textbf{0.682}} & \sethlcolor{tabcolor5}\hl{\textbf{0.663}} & \sethlcolor{tabcolor5}\hl{\textbf{0.737}} & \sethlcolor{tabcolor5}\hl{\textbf{0.759}} & \sethlcolor{tabcolor5}\hl{\textbf{0.734}}\\
        \bottomrule
    \end{tabular}}
    \captionof{table}{Evaluation of language coherence. The ``Win'' column indicates the ratio of cases where ID wins.}
    \label{tab:eval_sc}
\end{minipage}
